Broadband Spectral Analysis of 1ES2344+514: A Multi-epoch study

We present the results of the multi-epoch broadband spectral study of 1ES 2344+514 and study the evolution of physical parameters. We used nearly simultaneous data obtained from 2017 June 6 to 2022 August 6 (MJD 57910 -- 59797) in optical, UV, X-ray and $\gamma$-ray wavebands from various instruments including Swift-UVOT, Swift-XRT, NuSTAR, AstroSat (SXT and LAXPC), Fermi-LAT, and TeV flux from MAGIC. During 2017 July, 1ES 2344+514 appeared to be in the highest flaring state compared to other periods. We used the 0.5 -- 7.0 keV and 3.0 -- 20.0 keV data, respectively, from SXT and LAXPC of AstroSat and also 0.3 -- 8.0 keV and 3.0 -- 79.0 keV data, respectively, from Swift-XRT and NuSTAR. A joint fit between SXT and LAXPC, and between Swift-XRT and NuSTAR has been done for constraining the synchrotron peak. A clear shift in the synchrotron peak has been observed, which included 1ES 2344+514 in the HSP BL Lac family. A `harder-when-brighter' trend is observed in X-rays, and the opposite trend, i.e., `softer-when-brighter', is seen in the $\gamma$-rays. The multi-epoch broad-band spectral energy distributions (SEDs) of this source were built and studied to get an idea of the radiation processes. The SEDs were fitted using a steady-state leptonic one-zone synchrotron+SSC model, and the fitted parameters of the emission region are consistent with those of other TeV BL Lacs. In this study, we found a weak correlation tendency between bolometric luminosity and magnetic field (B), as well as between bolometric luminosity and the break Lorentz factor ($\gamma_{break}$).

==> readme <==
Dear Colleagues: 

The final publication layout will be produced by using raa.cls. 
Therefore, we strongly encourage you to prepare your LaTeX manuscript 
with this class file. Please unpack raa-package.tar.gz, it includes 

raa.cls        ---- RAA macro class file for LaTeX2e 
sample.tex     ---- a sample file using raa.cls (LaTeX source) 
sample.ps      ---- the PS file created by sample.tex in referee format  
sample.pdf     ---- the PDF file created by sample.tex in referee format  
readme         ---- this file  
f?.eps         ---- three demo figures used in the LaTeX template source
sample2.tex    ---- a sample file for using raa.bst
sample2_fig?.eps -- two demo figures used in sample2.tex
sample2.pdf    ---- the PDF file created by sample.tex in referee format
sample2.bbl    ---- bibliography file using by sample2.tex
bibtex.bib     ---- an example for bibtex file

natbib.sty     ---- This package reimplements the LaTeX \cite command
natnotes.pdf   ---- Brief reference sheet for Natbib (pdf)
raa.bst        ---- Bibliography style file 

Hope you enjoy the use of this macro. Your suggestions and comments are 
highly welcome. Thanks.

Editorial Office
E-mail:  raa@raa-journal.org

